Evaluating the faithfulness of PDF uncertainties in the presence of inconsistent data

We critically assess the robustness of uncertainties on parton distribution functions (PDFs) determined using neural networks from global sets of experimental data collected from multiple experiments. We view the determination of PDFs as an inverse problem, and we study the way the neural network model tackles it when inconsistencies between input datasets are present. We use a closure test approach, in which the regression model is applied to artificial data produced from a known underlying truth, to which the output of the model can be compared and its accuracy can be assessed in a statistically reliable way. We explore various phenomenologically relevant scenarios in which inconsistencies arise due to incorrect estimation of correlated systematic uncertainties. We show that the neural network generally corrects for the inconsistency except in cases of extreme uncertainty underestimation. When the inconsistency is not corrected, we propose and validate a procedure to detect inconsistencies.

==> sec-approach.tex <==
\section{Closure tests with inconsistent data}
\label{sec:approach}

The fundamental premise of closure testing involves taking a
given PDF set that acts as a proxy for the {\it true} proton structure
and a given theoretical model computed at a given perturbative
accuracy used to computed the partonic cross sections and generate a
set of artificial data points.
Such data points can be seen as ideal, in the sense
that they possess known statistical properties, exhibit no internal
inconsistencies, and are fully compatible with the theoretical model
employed in their generation. As a result, in a standard closure test, the expectation is to 
faithfully reproduce the underlying PDF within the correct margins of uncertainty.

In this section we present the next step in the landscape of closure tests: \textit{inconsistent} closure tests.
We start by in Sect.~\ref{subsec:approach} by properly defining what we mean by \textit{inconsistent} and how we practically inject
experimental inconsistencies in the set of artificial data.
In Sect.~\ref{subsec:setup} we define the practical settings of the implementation.

\subsection{Approach}
\label{subsec:approach}
%
As we mentioned in Sect.~\ref{sec:intro} inconsistencies of experimental nature arise when
some experimental uncertainties are either underestimated or entirely overlooked. As a result the nominal
standard deviation is smaller than the {\it true} one and, given the correlated multi-dimensional nature of measurements,  correlations might be miscalculated, thus causing tension between different experimental observations.
%
Although experimentalists are extremely careful in precisely
estimating the uncertainties associated with the measurements, in the
presence of highly correlated data with small statistical
uncertainties, the correct estimation of systematic uncertainties and
their correlation is a highly non-trivial exercise.
As such the exploration of the results of closure tests in the presence of {\it inconsistencies} of
experimental origin brings the closure test set-up closer to
real-world situations.

In order to formalise the definition of inconsistency in the context of a NNPDF-like closure test we write explicitly the experimental
covariance matrix $C_Y$ in the definition of $C$ given in Sect.~\ref{subsec:nn},
\begin{align}
\nonumber
    \left(C\right)_{ij} & = \delta_{ij} \sigma_i^{(\rm uncorr)} \sigma_j^{(\rm uncorr)} + \sum_{m=1}^{N_{\rm mult}} \sigma_{i,m}^{(\rm mult)} \sigma_{j,m}^{(\rm mult)} D_i D_j
     + \sum_{k=1}^{N_{\rm add}} \sigma_{i,k}^{(\rm add)} \sigma_{j,k}^{(\rm add)}  +  \left(C_{\rm th}\right)_{ij}
    \label{eq:experimental covmat}
\end{align}
where $\sigma_i^{\rm (uncorr)}$ denote the uncorrelated systematics, $\sigma_i^{(\rm mult)}$ the
correlated multiplicative systematics,  and $\sigma_i^{(\rm add)}$ denote the correlated additive systematics.
%
%In the context of HEP data, under the assumption of normally distributed experimental data, the published
%central value $y_0$ and the published experimental covariance matrix simply give us statistical information
%regarding the distribution of the {\it true} value of a given function or parameter:
%\begin{equation}
 %   f \sim \mathcal{N}(y_0,C_{Y}).
%\end{equation}
% MUB: we have already discussed the NNPDF methodology and cited Mark's paper
%The NNDPF methodology for fitting makes use of this information employing the Monte Carlo replica method as already described (si cita articolo MC/Bayesian di Mark Maeve etc?), and the closure test checks whether the methodology deploys faithful uncertainties.

In order to mimic the situation in which the experimental part of the
total covariance matrix has been unfaithfully estimated, we introduce
$C_{1}$ and $C_{2}$, denoting the covariance matrix used to generate
$L_1$ and $L_2$ data respectively, {\it i.e.},
\begin{itemize}
        \item Level-1 data: $L_1 = L_0 + \eta$, $\eta \sim \mathcal{N}(0,C_1)$ .
        \item Level-2 data: $L_2^{(k)} = L_1 + \epsilon^{(k)}$, $\epsilon^{(k)} \sim \mathcal{N}(0,C_2)$, $k = 1,...,N_{\rm reps}$ .
\end{itemize}
In a consistent closure test the covariance matrices for the generation of $L_1$ and $L_2$ data coincide:
\begin{align}
    C_{1} = C_{2} = C.
\end{align}
In a closure test in which we inject experimental inconsistencies instead
\begin{align}
    C_{1} = C \;\;{\rm and}\;\;C_{2} = C(\lambda),
\end{align}
with
\begin{align}
  \left[C(\lambda)\right]_{ij} & = \delta_{ij} \sigma_i^{(\rm uncorr)} \sigma_j^{(\rm uncorr)} + \sum_{m=1}^{N_{\rm mult}}
                                 \lambda_{i,m}^{\rm (mult)} \sigma_{i,m}^{(\rm mult)} \lambda_{j,m}^{\rm (mult)} \sigma_{j,m}^{(\rm mult)} D_i D_j \\
    & + \sum_{k=1}^{N_{\rm add}} \lambda_{i,k}^{\rm (add)}\sigma_{i,k}^{(\rm add)} \lambda_{j,k}^{\rm (add)}\sigma_{j,k}^{(\rm add)}  +  \left(C_{\rm th}\right)_{ij} ,
\end{align}
where in principle the rescaling factor $\lambda_{i,m}^{\rm (mult)},
\lambda_{i,k}^{\rm (add)}\in [0,1]$ can be different for each datapoint
and for each systematic uncertainty.
%
It is clear that these changes mimic a miscalculation in the published experimental covariance matrix: we generate the
$L_2$ data replica \textit{as if} $C$ had underestimated correlations
tuned by the $\lambda$ factor with respect to the true covariance
matrix $C_{1}$, thus potentially shifting the central values from the underlying truth.

To visualise the effect of rescaling multiplicative systematics by a factor $\lambda<1$, in Fig.~\ref{fig:data_generation} we show a simple
$2D$ case to visualise what happens when tuning the $\lambda$
parameter. In this illustrative example $X$ and $Y$ simply denote the
two observables, whose underlying true values are $X=0,\, Y=0$. The
covariance matrix is given by
%
\begin{equation}
C(\lambda) =
\begin{pmatrix}
  1.1 & \lambda \\
  \lambda & 1.1
\end{pmatrix}.
\end{equation}
%The actual values do not really matter in this case, this is just to
%show graphically what happens as we tune the inconsistency.
In this example $\lambda = \text{Var}(X,Y)$ and it plays the role of the tuned correlated uncertainties.
%
\begin{figure}[htb]
    \centering
  \includegraphics[width=0.48\textwidth]{images/final/New_consistent.pdf}
  \includegraphics[width=0.48\textwidth]{images/final/New_inconsistent.pdf}
  \caption{Left panel: the red dots are the $L_1$ generated
    instances, while the confidence ellipses show the distribution of
    the $L_2$ data, conditional on the respective $L_1$ data instances. The
    $L_1$ instances are generated according to a multi Gaussian centred
    in the underlying true value (the origin in this plot) with the
    same confidence ellipses as the $L_2$ ones. Right panel: the $L_1$
    data are generated according to a multi Gaussian with same ellipse
    as the consistent case, but $\lambda$ is set to $0$ to show the complete loss of correlation information.}
  \label{fig:data_generation}
\end{figure}
%
%Recalling the above definition for $C_{1}$ and $C_{2}$ we can clearly
%see that these are high-dimensional block matrices, where their
%dimensionality is fixed by the \textit{number of different training
%  data} we are using. The blocks, on the other hand, are defined by the correlated data points, which are 
%usually aggregated within different experiments (i.e., there is no inter-experiment correlation).
%
%
%From a practical point of view one has to choose the following things to properly introduce an inconsistency and deploy an inconsistent closure test: the set of datapoints in which an inconsistency is injected, the value(s) of $\lambda$ associated to each correlated systematics, and the strenghts of the inconsistency, which is maximal as $\lambda_{m,k}=0$ and
%zero as $\lambda_{m,k}=1$.
%In the analyses that will be presented in Sect.~\ref{sec:results} we will set $\lambda_k^{\rm (add)}=1$ for all additive systematics uncertainties $k$, while we will set $\lambda_m^{\rm (mult)}=\lambda<1$ for all multiplicative systematics uncertainties $m$.
%
%Once the setup for the data generation is defined, one can deploy as per usual a closure testing procedure.
%It is clear that we expect some change in the outcome that dependes on the level of inconsistency that is injected in the
%synthetic data.
Scanning $\lambda$ from 1, which reduces to the usual closure test with consistent data, to $\lambda=0$, which
corresponds to the maximum level of inconsistency in our set-up, we
can observe that, as $\lambda$ decreases, the information on
correlations between observables is lost and the ellipses change shape
until they become circles. 

This simple example shows us how the changes in $R_{bv}$ as an
experimental inconsistency injected in the artificial data is more severe indicate
to which measure a given experimental inconsistency may spoil the faithfulness of the PDF uncertainties.
We can assess whether the fitting methodology {\it absorbs} or {\it flags} the
experimental inconsistency that we artificially inject.

\subsection{Setup}
\label{subsec:setup}

In this Section we summarise the common settings that we use to
produce the results presented in Sect.~\ref{sec:results}.

First of all the $L_1$ data are generated by using as {\it underlying law} $f$ one of the
replicas of the {\tt NNPDF4.0} set, the same as the one used in
Sect.~5 of Ref.~\cite{DelDebbio:2021whr}, in which a single replica
was drawn randomly from a previous NNPDF
fit to experimental data. This has generally more structure than the final central PDF and it
is therefore a more general choice than any final central fit. 
In principle any function could be used as underlying law, however
it makes sense to use a realistic input.

We perform $N_{\rm fits}=25$ closure tests each of which done on a different, randomly sampled, $L_1$ type of noise and consisting of
$N_{\rm reps}=100$ replicas each. This choice, in particular, is motivated by previous studies~\cite{NNPDF:2021njg}.

In each of the cases discussed in Sect.~\ref{sec:results} we will
specify the set of datapoints affected by inconsistencies, 
the value(s) of $\lambda$ associated to each correlated systematics, and the strenghts of the inconsistency,
which is maximal as $\lambda=0$ and zero as $\lambda=1$.
Across the analyses that we present in the next sections we set $\lambda_{i,k}^{\rm (add)}=1$ for all additive systematic
uncertainties $k$, while we set $\lambda_{i,m}^{\rm (mult)}=\lambda\le 1$ for all multiplicative systematic uncertainties $m$ of some chosen datasets.
Note that this type of systematic represents the majority of the
systematics in the HERA and LHC data that we consider. Some of these
uncertainties are correlated not only across different kinematic
binnings of the same measurement, but also across different datasets
within the same experiment. For example, several ATLAS datasets are correlated with each other through the luminosity uncertainty.

Whenever we show the results for the ratio bias-variance obtained using a
PCA regularisation of the covariance matrix in the
space of PDFs we opt for an Explained Variance Ratio (EVR) of 0.99
across all datasets.  As explained in Sect.~\ref{subsec:comp} this selection allows us to retain maximum
information from the samples while simultaneously regularising the covariance matrix.

